All You Need is DAG

We present DAG-Rider, the first asynchronous Byzantine Atomic Broadcast protocol that achieves optimal resilience, optimal amortized communication complexity, and optimal time complexity. DAG-Rider is post-quantum safe and ensures that all messages proposed by correct processes eventually get decided. We construct DAG-Rider in two layers: In the first layer, processes reliably broadcast their proposals and build a structured Directed Acyclic Graph (DAG) of the communication among them. In the second layer, processes locally observe their DAGs and totally order all proposals with no extra communication.

==> sections/enhancements.tex <==
\section{Enhancements}


\subsection{DAG can implement the global perfect coin}
No other crypto other than that. Adversary assumption are only for
liveness. Safety is fine due to the signature schema. 


\subsection{Given a BC service, we only need 2f+1 process in the DAG}
No equivocation 

\subsection{Lowering the amortized complexity}

The current protocol has an amortized quadratic cost per transactions. This meets the performance of VABA, however, Dumbo showed how the use of error-correcting codes 
can reduce the amortized cost to linear. This idea is also applicable to our system. In order to get linear amortized cost per transaction we can substitute the vanilla reliable broadcast with the Asynchronous Verifiable Information Dispersal of Cachin and Tessaro. Using this we can reliably disperse the $O(n)$ blocks with a cost of $O(n^2logn)$  which would lead to an amortized cost of O(nlogn) per transaction. Fortunately AVID can support a larger batch size of $O(nlogn)$ with the same cost, hence by slightly increasing the number of transactions per bloc to $O(nlogn)$ we can get the amortized cost per transaction done to the optimal $O(n)$ matching Dumbo's performance. 


\subsection{Transaction Load Characteristics}

One natural question is how are transactions distributed to parties. If clients sends transactions to everyone then it is highly likely that all blocks from different nodes will contain the same transactions, hence reducing the true throughput by $O(n)$ compared to the apparent throughput we calculate. By adding probabilistic guarantees and economic incentives we instead reduce this redundancy only to a constant factor. First, in a blockchain system we can add an explicit payment to the source node when the client sends the transactions, hence replicating the transaction will also multiply the fee and make the client consider being more frugal. Additionally although to get deterministic guarantees the client needs to send to $f+1$ nodes the transaction, we can get strong probabilistic guarantees with a constant number of copies (e.g., $4$ random copies give a 99\% chance of including an honest node). As a result we let the client decide between economic cost (each copy costs) and latency (the more copies the better the chance a transaction gets included.)


==> sections/fairness.tex <==
\section{Fairness}
We consider a number of alternatives in the adversary's ability to control the correct processes' messages.
The different options we consider are described as follows:
\begin{description}
	\item[Full control] The adversary can schedule the timing and the order of the messages' arrivals times, regardless if the sender or the receiver is a correct processes or not.
	
	\item[Random arrival times] In this model the adversary has no control of the correct processes' messages' arrival times.
	When a correct process $p$ sends a message $m$ to another correct process at time $t$, the time until $m$'s delivery,  is randomly sampled from a sample space $\Omega$, i.e., $m$ will arrive at its destination by $t + \omega$, where $\omega \in \Omega$ was sampled at $t$ and is not known to any process in the system nor the adversary.
	Nevertheless, if the adversary corrupts $p$ before $m$'s arrival time, it can decide to drop $m$.
	
	\item [Mobile partial control] The adversary at any time during the run can control up to $k \leq 2f+1$ of the  correct processes' network and delay their messages arbitrarily. 
	The adversary, at its discretion, can choose which correct processes to delay throughout the execution, as long as in each point in time during the run this number is less than $k$. 
	Notice that for $k = 2f + 1$ this model is equivalent to a full control adversary.
	The arrival times of the correct process who are not under the adversary's control are randomly chosen in a similar way to the random arrival times option.
	
	
	\item[Random partial control] The adversary at any time during the run can control up to $k \leq 2f+1$ of the correct processes' network and delay their messages.
	When the adversary takes control of a correct proces $p$'s network, the length of that control time is randomly chosen from a sample space $\Omega_1$, after which the adversary looses control of $p$'s network for an amount of time which cannot be less than a random length of time chosen from a sample space $\Omega_2$.
	The arrival times of the correct process who are not under the adversary's control are randomly chosen in a similar way to the random arrival times option.
	
	
	\item[Random ordering] Let $M(t)$ be an ordered set of all the messages which were sent by correct processes before $t$ and did not arrive by $t$.
	When a correct process sends a message at time $t'$ it is added to $M(t')$ in a random place in the set which is randomly chosen from a sample space $\Omega$.
	When a message arrives at time $t$ it is removed from $M(t)$.
	
	At any time $t$ during the run, the adversary can choose to cause the first message in $M(t)$ to arrive, i.e., it can control the arrival times of messages, but cannot determine the order in which the messages are delivered.
	As in other asynchronous models, eventually the adversary has to deliver all the messages that were sent by correct processes, i.e., $\lim_{t \to \infty} \left| M(t) \right| = 0$.
\end{description}

\section{Problem Definition}

\begin{table}[t]
	\centering
	\caption{\textbf{Summary of the different network models and the fairness types.} A \cmark means that there exists an SMR algorithm that guarantees the fairness type in the network model, and an \xmark means an impossibility result on such an algorithm.}
	\begin{tabular}{ |c | c c c|} 
		\hline
		\textbf{Network Model} &\textbf{Complete Fairness} & \textbf{Partial Fairness} & \textbf{Eventual Fairness} \\
		\hline
		Full control & \xmark & \xmark & ? \\
		Random Arrival times & \cmark & \cmark & \cmark \\
		Mobile partial control & \xmark & \xmark & \cmark \\
		Random partial control & \xmark & ? & \cmark \\
		Random ordering & ? & ? & \cmark \\
		\hline
	\end{tabular}
	\label{tab:fairnessComparison}
\end{table}



%	\item[External validity] For any transaction $tx$ in the ledger $\textit{validate}(tx)$ returns true.
%	
%	\item[Progess/Liveness] The ledger $\mathcal{L}$ eventually adds more transactions, i.e., in an infinite run, $\mathcal{L}_i$ contains an infinite number of transactions.
%\end{description} 	

In addition to the properties above, we want to design a \emph{fair} SMR protocol.
In contradiction to the first three properties, fairness has been defined differently in different works such as~\cite{cachin2001secure,kelkar2020order} and also has a different meaning in a single-shot consensus protocol as opposed to multiple-shot SMR.
Intuitively, in a consensus protocols, most works who require external validity, define fairness as the probability that the decision reached will originate from a correct process to be at least as the chance that it originated from the adversary.
In an SMR protocols, multiple decisions are reached.
Therefore, it makes more sense to define fairness as a global property over the entire ledger.

Since in an infinite run, an SMR protocol commits an infinite number of decisions, we give a few definitions to the notions of fairness.
Let $\mathcal{L}_i^f[k]$ be the set of transactions in $\mathcal{L}^f[k]$ that were proposed by $p_i$.
In addition, let $\textit{proposer}(tx)$ be the process which proposed transaction $\textit{tx}$.

With this we define a completely fair SMR protocol, which intuitively means that for each committed transaction in the ledger, each correct process has an equal shot to propose that transaction.

\begin{definition} [Completely fair SMR protocol]
	An SMR protocol is \emph{completely fair} if for any  $k \in \mathbb{N}$ and for any correct process $p_i \in \Pi$ the following holds:
	\begin{equation*}
		\Pr \left[ \textit{proposer}(\mathcal{L}[k]) = p_i \right] \geq 1/n
	\end{equation*}
\end{definition}

Next, we define an eventually fair SMR protocol.
This fairness definition ensures that in an infinite run all correct processes have an equal opportunity to commit transactions to the ledger.

\begin{definition} [Eventually fair SMR protocol]
	An SMR protocol is \emph{eventually fair} if for any correct process $p_i \in \Pi$
	\begin{equation*}
		\lim_{k \to \infty} \mathcal{L}^f_i \left[ k \right] / \mathcal{L}^f\left[ k \right]  \geq 1/n
	\end{equation*}
\end{definition}

Lastly, we define a partial fair SMR protocol:

\begin{definition} [Partially fair SMR protocol]
	An SMR protocol is \emph{partially fair} if for any correct process $p_i \in \Pi$ there exists a bound $k' > 0$ such that 
	\begin{equation*}
		\mathbb{E} \left[ \left( \mathcal{L}^f_i[k+k'] \setminus  \mathcal{L}^f_i[k]  \right) / \left(  \mathcal{L}^f[k+k'] \setminus \mathcal{L}^f[k] \right)\right] \geq 1/n
	\end{equation*}
\end{definition}

Another notion of fairness, sometine




\section{Results}

\begin{algorithm*}[t]
	\caption{Networking model, will work between the consensus layer and the networking. Will probably be good for random partial control/random ordering for partial and eventual fairness.}
	\label{alg:DAGabstraction}
	
	\begin{algorithmic}[1] 
		
		\item[]
		\Statex \textbf{Local Variables:}
		\StateX $r \gets 1$ \Comment{round number}
		\StateX $k \gets 0$ \Comment{Number of messages received, reset after each $2f+1$ for each round}
		\StateX $\textit{round\_processes}$ 
		
		
		\item[]
		\Upon{receiving a valid message $m$ for round $r'$ from process $q$}
		\If{$r \neq r'$}
		\State break
		\EndIf
		\If{$q \in \textit{round\_processes} $or $\textit{round\_processes} = \emptyset$}
		\State $\textit{round\_processes} \gets \textit{round\_processes} \setminus q$
		\State $k \gets k+1$
		\State $\textit{deliver}(m)$
		\EndIf
		\If{$\left| \textit{round\_processes} \right| \leq f$}
		\State $\textit{round\_processes} \gets \emptyset$
		\EndIf
		\If{$k \geq 2f+1$}
		\State $\textit{round\_processes} \gets \text{randomly choose } 2f +1 \text{ processes from } \Pi$
		\State $k \gets 0$
		\State $r \gets r+1$
		\EndIf
		\EndUpon
		
	\end{algorithmic}
\end{algorithm*}

We start by showing an impossibility result. 
It shows that in the standard asynchrony model where the adversary has full control of the arrival times of correct processes' messages, complete fairness or even partial fairness cannot be guaranteed.
Intuitively this is because the adversary can delay some of the correct processes' messages without any limitations (as lont as they are eventually delivered).
This is different from the eventual synchrony model in the sense that there the adversary can only delay the arrival times of messages after GST until a certain upper bound.
We will show that by limiting the adversary's power in the asynchrony model, e.g., by determining that the arrival times of the correct processes' messages is determined randomly, fairness can be guaranteed.

\begin{lemma}
	There does not exist an SMR algorithm in the full control asynchronous model that guarantees full fairness or partial fairness.
\end{lemma}
